Optimal Regulation and Investment Incentives in Financial Networks

We examine optimal regulation of financial networks with debt interdependencies between financial firms. We first show that firms often have an incentive to choose excessively risky portfolios and overly correlate their portfolios with those of their counterparties. We then characterize how optimal regulation depends on a firm's financial centrality and its available investment opportunities. In standard core-periphery networks, optimal regulation depends non-monotonically on the correlation of banks' investments, with maximal restrictions for intermediate levels of correlation. Moreover, it can be uniquely optimal to treat banks asymmetrically: restricting the investments of one core bank while allowing an otherwise identical core bank (in all aspects, including network centrality) to invest freely.

==> NS_example.tikz.tex <==
\begin{tikzpicture}[scale=8]
\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36};
\definecolor{afblue}{rgb}{0.36, 0.54, 0.66};
\foreach \Point in {(0,0), (0,3)}
\draw[fill=chestnut] \Point circle (0.2);
\foreach \Point in {(-2,1.5), (3,3), (3,0)}
\draw[fill=chestnut!60] \Point circle (0.2);
\foreach \Point in {(-4,1.5), (-4,2.6), (-4,0.4), (-4,0.9)}
\draw[fill=afblue!40] \Point circle (0.15);
\draw[->, thick] (0.1,0.5) to (0.1,2.5) ;
\draw[<-, thick] (-0.1,0.5) to    (-0.1,2.5) ;
\draw[->, thick] (0.5,-0.1) to  (2.5,-0.1) ;
\draw[<-, thick] (0.5,0.1) to  (2.5,0.1) ;
\draw[<-, thick] (0.5,2.9) to  (2.5, 2.9) ;
\draw[->, thick] (0.5,3.1) to (2.5, 3.1) ;
\draw[<-, thick] (0.4,0.3) to  (2.7, 2.6) ;
\draw[->, thick] (0.3,0.45) to  (2.6, 2.75) ;
\draw[<-, thick] (2.6,0.3) to  (0.3, 2.6) ;
\draw[->, thick] (2.7,0.45) to  (0.4, 2.75) ;
\draw[<-, thick] (-0.4,0.3) to  (-1.7, 1.1) ;
\draw[->, thick] (-0.3,0.45) to  (-1.6, 1.25) ;
\draw[<-, thick] (-0.4,2.7) to  (-1.7, 1.9) ;
\draw[->, thick] (-0.3,2.55) to  (-1.6, 1.75) ;

\draw[->, thick] (-2.3, 1.8) to  (-3.7, 2.5) ;
\draw[->, thick] (-2.3, 1.3) to  (-3.7, 0.5) ;
\draw[->, thick] (-2.38, 1.41) to  (-3.7, 0.95) ;
\draw[->, thick] (-2.4, 1.5) to  (-3.7, 1.5) ;

\node at (-3.6,2.1)  {\small $\vdots$};

%\draw[<-, thick] (-2.5,0) to node [ above, sloped]  {$1$} (-0.5,0) ;
%\draw[<-, thick] (-2.5,3) to node [ above, sloped]  {$1$} (-0.5,3) ;
%\draw[<-, thick] (5.5,0) to node [ above, sloped]  {$1$} (3.5,0) ;
%\draw[<-, thick] (-5.5,0) to node [ above, sloped]  {$1$} (-3.5,0) ;
%\draw[<-, thick] (-5.5,3) to node [ above, sloped]  {$1$} (-3.5,3) ;
%\draw[<-, thick] (8.5,0) to node [ above, sloped]  {$1$} (6.5,0) ;
%\draw[<-, thick] (5.5,3) to node [ above, sloped]  {$1$} (3.5,3) ;
%\draw[<-, thick] (8.5,3) to node [ above, sloped]  {$1$} (6.5,3) ;
%
%\foreach \Point in {(-7,0), (-7,3), (10,0), (10,3)}
%\node at \Point  {\small depositors};



  \end{tikzpicture}  

==> contracts.tikz.tex <==
\begin{tikzpicture}
\draw[->, thick] (0,0)--(5,0) node[right, below]{$V_j$};
\draw[->, thick] (0,0)--(0,3) node[above, left]{$f_{ij}$};
\draw[cyan!50!black,thick] (0,0) -- (4.8,1.4);
\draw[red!50!black,thick] (0,0) -- (1.5,1.1);
\draw[red!50!black,thick] (1.5,1.1) -- (4.8,1.1);
\draw[green!50!black,thick] (0,0) -- (4,0);
\draw[green!50!black,thick] (4,0) -- (4.8,0.8);
\draw (3.3,0) node[anchor=south, green!50!black] {\small call option};
\draw (3,0.4) node[anchor=south, cyan!50!black] {\small equity};
\draw (2.9,1.1) node[anchor=south, red!50!black] {\small debt};

  \end{tikzpicture}  

==> contracts2.tikz.tex <==
\begin{tikzpicture}
\draw[->, thick] (0,0)--(5,0) node[right, below]{$V_j$};
\draw[->, thick] (0,0)--(0,3) node[above, left]{$f_{ij}$};
\draw[cyan!50!black,thick] (0,2) -- (1,2);
\draw[cyan!50!black,thick] (1,0) -- (4.8,0);
\draw (0.5,2.1) node[anchor=south, cyan!50!black] {\small CDS};
\draw[red!50!black,thick] (0,1.3) -- (1.3,0);
\draw[red!50!black,thick] (1.3,0) -- (4.8,0);
\draw (0.8,1.2) node[anchor=south, red!50!black] {\small put option};

  \end{tikzpicture}  

==> core_peri_example.tikz.tex <==
\begin{tikzpicture}[scale=8]
\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36};
\definecolor{afblue}{rgb}{0.36, 0.54, 0.66};
\foreach \Point in {(0,0), (0,3), (3,3), (3,0)}
\draw[fill=chestnut] \Point circle (0.2);
\foreach \Point in {(-3,0), (-3,3), (6,0), (6,3)}
\draw[fill=afblue!40] \Point circle (0.2);
\draw[->, thick] (0.1,0.5) to (0.1,2.5) ;
\draw[<-, thick] (-0.1,0.5) to    (-0.1,2.5) ;
\draw[->, thick] (3.1,0.5) to (3.1,2.5) ;
\draw[<-, thick] (2.9,0.5) to   (2.9,2.5) ;
\draw[->, thick] (0.5,-0.1) to  (2.5,-0.1) ;
\draw[<-, thick] (0.5,0.1) to  (2.5,0.1) ;
\draw[<-, thick] (0.5,2.9) to  (2.5, 2.9) ;
\draw[->, thick] (0.5,3.1) to (2.5, 3.1) ;
\draw[<-, thick] (0.4,0.3) to  (2.7, 2.6) ;
\draw[->, thick] (0.3,0.45) to  (2.6, 2.75) ;
\draw[<-, thick] (2.6,0.3) to  (0.3, 2.6) ;
\draw[->, thick] (2.7,0.45) to  (0.4, 2.75) ;

\draw[<-, thick] (-2.5,0) to node [ above, sloped]  {$1$} (-0.5,0) ;
\draw[<-, thick] (-2.5,3) to node [ above, sloped]  {$1$} (-0.5,3) ;
\draw[<-, thick] (5.5,0) to node [ above, sloped]  {$1$} (3.5,0) ;
\draw[<-, thick] (-5.5,0) to node [ above, sloped]  {$1$} (-3.5,0) ;
\draw[<-, thick] (-5.5,3) to node [ above, sloped]  {$1$} (-3.5,3) ;
\draw[<-, thick] (8.5,0) to node [ above, sloped]  {$1$} (6.5,0) ;
\draw[<-, thick] (5.5,3) to node [ above, sloped]  {$1$} (3.5,3) ;
\draw[<-, thick] (8.5,3) to node [ above, sloped]  {$1$} (6.5,3) ;

%\draw[->, thick] (0.1,0.5) to (0.1,3.5) ;
%\draw[<-, thick] (-0.1,0.5) to  node[midway,fill=white] {$\, D$}  (-0.1,3.5) ;
%\draw[->, thick] (0.5,0.1) to  (2.9,1.6) ;
%\draw[<-, thick] (0.3,0.3) to node [ midway, below = -0.8em]  {\colorbox{white}{$D$}} (2.7,1.8) ;
%\draw[<-, thick] (0.4,4) to  (2.8, 2.5) ;
%\draw[->, thick] (0.3,3.7) to node [midway, above=-0.7em]  {\colorbox{white}{$D$}}  (2.7, 2.2) ;
%\draw[<-, thick] (-2.5,0) to node [ above, sloped]  {$\bar{d}$} (-0.5,0) ;
%\draw[<-, thick] (-2.5,4) to node [ above, sloped]  {$\bar{d}$} (-0.5,4) ;
%\draw[<-, thick] (5.5,2) to node [ above, sloped]  {$\bar{d}$} (3.5,2) ;
%\draw[<-, thick] (-5.5,0) to node [ above, sloped]  {$\underline{d}$} (-3.5,0) ;
%\draw[<-, thick] (-5.5,4) to node [ above, sloped]  {$\underline{d}$} (-3.5,4) ;
%\draw[<-, thick] (8.5,2) to node [ above, sloped]  {$\underline{d}$} (6.5,2) ;
\foreach \Point in {(-7,0), (-7,3), (10,0), (10,3)}
\node at \Point  {\small depositors};



  \end{tikzpicture}  
